Robust Graph Representation Learning via Predictive Coding

Predictive coding is a message-passing framework initially developed to model information processing in the brain, and now also topic of research in machine learning due to some interesting properties. One of such properties is the natural ability of generative models to learn robust representations thanks to their peculiar credit assignment rule, that allows neural activities to converge to a solution before updating the synaptic weights. Graph neural networks are also message-passing models, which have recently shown outstanding results in diverse types of tasks in machine learning, providing interdisciplinary state-of-the-art performance on structured data. However, they are vulnerable to imperceptible adversarial attacks, and unfit for out-of-distribution generalization. In this work, we address this by building models that have the same structure of popular graph neural network architectures, but rely on the message-passing rule of predictive coding. Through an extensive set of experiments, we show that the proposed models are (i) comparable to standard ones in terms of performance in both inductive and transductive tasks, (ii) better calibrated, and (iii) robust against multiple kinds of adversarial attacks.

==> FINAL arXiv- Robust Graph Representation Learning via Predictive Coding/Sections/Appendices.tex <==
\appendix

\begin{comment}
\section{Predictive Coding}
In both human and robotic learning, it entails the process of credit assignment, or identifying the steps in the processing chain that lead to an incorrect outcome. Understanding how the brain deals with the credit assignment issue is crucial for the fields of neuroscience and artificial intelligence. Many recent studies have looked to backpropagation, a staple of modern machine learning, as the answer\cite{lillicrap2020backpropagation}. However, the brain's ability to do backpropagation has been questioned, and it has been proposed that the brain's natural approach to learning may be more effective in terms of both time and energy optimization \cite{tsividis2017human}. Predictive coding mechanism has presented itself as an excellent candidate as is capable training neural networks through energy minimization and has been able to explain several brain functions.


Predictive coding is an influential theory of information processing in the brain. Predictive coding proposes that the brain has a world model or many world models in distinct brain areas where each model is a generative model that captures the cause of sensory input. New sensory inputs are then mapped to recognised causes. Minimizing the discrepancy between sensory data and predicted sensory inputs aids in determining which of multiple possible explanations best matches existing sensory data.

This idea has manifested itself independently in various areas and there are a number of distinct algorithms that have been proposed to realise it. In signal processing, linear predictive coding (LPC) was originally used in audio and speech processing for signal restoration, interpolation, compression and recognition \cite{spratling2017review}. LPC was initially employed in neuroscience to describe the function of the retina \cite{laughlin1990coding}, such as efficient coding, redundancy reduction, and normalisation. Later, numerous studies expanded on the notion of LPC to neural network based architecture to describe various cortical processes in the brain \cite{rao1999predictive, spratling2008predictive, friston2009free}. 

The training and inference mechanisms of predictive coding networks(PCNs) is in Appendix~\ref{sec:pc_formulation_sec}.

\section{Predictive Coding vs Back-propagation}

This section examines the differences between the backpropagation algorithm, the leading algorithm used to train artificial neural networks (ANNs), and inference learning (IL), which is one of the major method used to train predictive coding networks(PCNs).


\subsubsection{Training ANNs with BP}


% - Include a pc training algorithm in the background

A layer of an artificial neural network\cite{rumelhart1986learning} consists of a number of value nodes that mimic neurons. To further highlight the connection to PCNs, we invert the layer numbering scheme, assigning $0$ to the output layer and $l_{max}$ to the input layer (see \cite{song2020can} for additional details). Let nodes at $l^{th}$ layer be indicated by $\mathbf{h^l}$ vector, and for simplification we ignore the bias values. Then, the activation of $i$ neuron in in layer $l$ is calculated as follows:

\begin{equation}
\label{eqn:equ1}
  h_{i}^{l}=\sum_{j=1}^{|h^{l+1}|} w_{i, j}^{l+1} f\left(h_{j}^{l+1}\right)  
\end{equation}
where  $w_{i, j}^{l+1}$ denotes the synaptic weight connecting $l^{th}$ to ${l+1}^{th}$ layer.




\textbf{Learning}: Given the input vector $\mathbf{x}$ and true label vector $\mathbf{y}$, $\mathbf{h^{l_max}}$ is fixed to input vector $\mathbf{x}$ (i.e. $\mathbf{h^{l_max} = x}$). The output of the layer values are obtain through iterative application of Equation~\ref{eqn:equ1}, then the prediction error, E, is calculated using an objective function,  $\mathcal{L}$ (the most common loss function for classification and regression tasks are cross entropy and mean-squared error, respectively):


\begin{equation}
E=\mathcal{L}(\mathbf{y, h^0})
\end{equation}

Back-propagation algorithm\cite{rumelhart1986learning} essentially works by propagating the error gradient sequentially backward from the output layer through all network layers and utilises gradient descent algorithm to update the synaptic weight. The gradient with respect to a weight parameter,$w_{i, j}^{l+1}$, in layer ${l+1}$ is given by the following:

$$
\Delta w_{i, j}^{l+1}=-\eta \cdot \partial E / \partial w_{i, j}^{l+1}
$$

where $\eta$ denotes the learning rate. $i$ and $j$ subscripts represent in neurons in layer $l+1$ and $l$ respectively. 





\textbf{Prediction}: Given the input vector $\mathbf{x}$, $\mathbf{h^{l_max}}$ is fixed to input vector $x$ (i.e. $\mathbf{h^{l_max} = x}$), then the feedforward of the input signal through the network happen by recursively applying Equation~\ref{eqn:equ1}(like in training mode) and prediction are indicated by the output layer $0$. The top of Figure~\ref{fig:pc_bp} showcase this process.


% \subsubsection{Training PCNs with using inference learning}
% \label{sec:pc_formulation_sec}
% The architecture and learning method of Predictive Coding Networks(PCNs) is different from ANNs and back-propagation as illustrated in Figure~\ref{fig:pc_bp}. Like ANNs, PCNs have values nodes and synaptic weights, however, each values nodes is associated with additional error node, and are optimised using inference learning algorithm(see Algorithm~\ref{alg:cap}). In PCN architecture, a values node $h^{l}_{i, t}$ denotes neural activity of neuron $i$ at layer $l$ at time $t$ with corresponding prediction-error nodes $\varepsilon^{l}_{i, t}$. Inference learning\cite{whittington2017approximation} entail inferring the values of the hidden node through energy minimization. Different variations of IL such as Z-IL, Fa-Z-IL have been developed to make IL more efficient and give it full autonomy during training\cite{song2020can}.

% \textbf{Learning}: Given the input vector $\mathbf{x}$ and true label vector $\mathbf{y}$, $\mathbf{h^{l_max}}$ is fixed to input vector $x$ (i.e. $\mathbf{h^{l_max} = x}$) and output layer is fixed to true label values (i.e. $\mathbf{h^{0} = y}$). Unlike ANN that propagate the activity of nodes as directly, PCNs propagates the error node values, $\varepsilon__{i, t}^{l} $, i.e., the difference between the value nodes and the prediction of the node, $h^{l}_{i, t}$ and $\mu^{l}_{i, t}$, respectively.

% \begin{equation}
% \label{eqn:error_update}
% \mu_{i, t}^{l}=\sum_{j=1}^{|\mathbf{h^{l+1}}|} w_{i, j}^{l+1} f\left(x_{j, t}^{l+1}\right) \text { and } \varepsilon_{i, t}^{l}=h_{i, t}^{l}-\mu_{i, t}^{l} \text {, }
% \end{equation}

% where  $w_{i, j}^{l+1}$ denotes the synaptic weight  beween  node $i$ at layer $l$ and node $j$ at layer $l+1$.

% \textbf{Energy Minimization}. As PCNs are energy-based models, the training happen through minimization of the global energy in each layer. Under the assumption of Gaussian distribution with identify covariance, the energy,$F_{t}$ function of PCNs can be derived simply as the sum of errors of prediction-error nodes in the network \cite{whittington2017approximation}:

% $$
% F_{t}=\frac{1}{2} \sum_{i, l}\left(\varepsilon_{i, t}^{l}\right)^{2}
% $$


% Minimizing this function brings each value node $h^{l}_{i, t}$ closer to its correct prediction. Inference, in this case, describes this process of reducing energy function, $Ft$,via tweaking $h_{i, t}^{l}$ to match $\mu_{i, t}^{l}$. This process is described by the following equation dynamics:

% \begin{equation}
% \label{eqn:x_update}
% \Delta h_{i, t}^{l}= \begin{cases}0 & \text { if } l=l_max \\ \gamma \cdot\left(-\varepsilon_{i, t}^{l}+f^{\prime}\left(h_{i, t}^{l}\right) \sum_{k=1}^{n^{l-1}} \varepsilon_{k, t}^{l-1} w_{k, i}^{l}\right) & \text { if } 0<l<l_max \\ \gamma \cdot\left(-\varepsilon_{i, t}^{l}\right) & \text { if } l=0,\end{cases}
% \end{equation}


% where $\gamma$ is the integration step

% Using to the Equation~\ref{eqn:x_update}, the value nodes are updated until convergence, or until inference steps reaches $T$ iterations. Following the inference step, a single weight update is executed to further reduce the residual errors $E$. Then, the weights, $W$, are modified in order to minimise the same objective function $F_t$, using the following equation:

% \begin{equation}
% \label{eqn:w_update}
% \Delta w_{i, j}^{l+1}=-\alpha \cdot \partial F_{t} / \partial w_{i, j}^{l+1}=\alpha \cdot \varepsilon_{i, t}^{l} f\left(h_{j, t}^{l+1}\right)
% \end{equation}

% This inference learning process is described in Algorithm~\ref{alg:cap}.



% \textbf{Prediction}. For acyclic fully-connected network, the prediction stage is similar to ANNs, which is simply a single feed-forward pass of sensory signals through the network. Because the output is usually unconstrained, the inference process optimise the weights so that error nodes decay to zero as $t \rightarrow \infty$. Thus, the values nodes, $h_{i, t}^{l}$, converge to the prediction values, $\mu_{i, t}^{l}$. For architecture with complex topologies, a inference process is necessary during prediction stage\cite{salvatori2022learning}.



% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{img/pc_bp_diagram.pdf}
%     \caption{Neural implementation of Back-propagation (top) and predictive coding (bottom). The blue lines refers to  Equation~\ref{eqn:equ1} and Equation~\ref{eqn:error_update} ANN and PCN, respectively,  and the red line refers to Equation~\ref{eqn:x_update} for PCN .}
%     \label{fig:pc_bp}
% \end{figure}


% \begin{algorithm}
% \caption{Learning one training pair ($x$, $y$) (presented for the duration T, i.e., inference steps) with IL (This algorithm was adapted from \cite{song2020can})}\label{alg:cap}
% \begin{algorithmic}[1]
% \Require $h_{0 \max }^l$ is fixed to $y, \bar{h}_0^0$ is fixed to $x$

% \For {\texttt{ t=0 \text { to } T} }
% \For {\texttt{each neuron i in each level l} }

% \State \texttt{Update $h_{i, t}^l$ to minimize $F_t$ using Equation~\ref{eqn:x_update}}
% \State \texttt{Update each $w_{i, j}^{l+1}$ to minimize $F_t$ using Equation~\ref{eqn:w_update}}

   

% \EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}


% \textbf{Biological plausibility}. In additional to the ability of predictive coding to explain many neuro-biological phenomena,  one of the attractive of predictive coding networks is that they rely on local computation which explain local plasticity of synaptic weights. In contrast to BP,  Eqs~\ref{eqn:error_update}, \ref{eqn:x_update}, and \ref{eqn:w_update} in IL rely on local information. An external signal is still required to terminate inference at time $t=T$ and initiate the weights update, thus the full autonomy required for biological plausibility is not fully realised. However, an extension of IL known as fully autonomous zero-divergent IL (Fa-Z-IL) realise full autonomy\cite{song2020can}.
\end{comment}



\section{Details on evaluation metrics}

In this section, we explain the metrics used in the main body of this work in more detail. We employ scalar quantification metrics, such as expected calibration error (ECE) and maximum calibration error, together with visual tools, such as reliability diagrams and confidence distribution histograms \citep{guo2017calibration} and classification margin diagrams \citep{dai2018adversarial} to evaluate model calibration.

The term `confidence calibration` is used to describe the ability of a model to produce probability estimations that are accurate reflections of the correct likelihood an event, which is imperative especially in real-world applications. Considering a $K$-class classification task, let  $X \in \mathcal{X}$ and $Y \in \mathcal{Y}=\{1, \ldots, K\}$ be input and true ground truth label random variables, respectively. Let $\hat{Y}$ denote a class prediction and $\hat{P}$ be its associated confidence, i.e. probability of correctness. We would like the confidence estimate $\hat{P}$ to be calibrated, which intuitively means that $\hat{P}$ represents a true probability. The perfect calibration can be described as follows:
%
\begin{equation}
\label{eqn:calibration}
    \mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)=p, \quad \forall p \in[0,1]
\end{equation}
%
\textbf{ECE} captures the notion of average miscalibration in a single number, and can be obtained by the expected difference between  accuracy and confiedence of the model: $
\underset{\hat{P}}{\mathbb{E}}[|\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)-p|]
$




\textbf{MCE} is much crucial in safety-, security-critical settings, as it quantifies worst-case expected miscalibration: $
\max _{p \in[0,1]}|\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)-p| .
$

\textbf{Reliability diagrams} are visual representation tools for model calibration as equation~\ref{eqn:calibration} is intractable because  $\hat{P}$ is a continuous random variable. They characterise the average accuracy level inside a points that feels into a given confidence level bin (see \cite{} for more details on formulation of the the above metrics).

\textbf{Classification margin} is simply the difference between the model output probability of the ground truth class and the model probability of the predicted most-likely class, i.e.,the probability of the best second class. Thus, this metric is between $-1$ and $1$, where values close to $-1$ indicate that a model is overconfident in wrong predictions and values closer to $1$ indicate that the model is confidence in its correct prediction. In our reported class margin diagrams,  we average these values over many samples and repeated trials with different random seeds to draw box-plot diagrams of our results. 


\section{Reproducibility}

We use standard splits on all datasets. We report the average results of 5 runs on different seeds; the hyper-parameters are selected using the validation set. Following the results from original papers on baseline models, we evaluate our model on 2 GNN layers. The models are trained for 300 epochs on citation graphs and 50 epochs on PPI. We also use Adam optimiser. The reported results on calibration analysis were performed on initial learning rate of 0.001 for both GCN and GPCN as it provided best performances for both models. For adversarial attacks, we set initial learning rate to 0.01 and epochs to 200 to compare our results to other works. For general performance experiment, we use grid search for hyper-parameters as described in Table~\ref{tab:hyperpar}. Inductive tasks were trained using GCN version of GraphSage \citep{hamilton2017inductive} with neighborhood sample size of 25 and 10 for first and second GNN layer, respectively (see \cite{hamilton2017inductive} for more details). 


Our experiments are performed using Pytorch Geometric library \cite{fey2019fast}. In order to do an extensive experiment, we build on GraphGym \cite{you2020design}, a research platform for designing and evaluating GNNs, and we seamlessly integrate it with predictive coding learning algorithm. In addition, we employ another Pytorch library for adversarial attacks and defenses known as Deeprobust \cite{li2020deeprobust} for various type of adversarial attacks we perform on graphs.



\subsection{Datasets}
\begin{table}[H]
    \caption{An overview of the data sets used in our experiments }\label{tab:datasets}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{*{7}{|c}|}\hline
    %   • &\multicolumn{8}{c|}{West Hebrides} \\
    %  \hline
    %  • & \multicolumn{2}{c|}{$H_{s}$} &\multicolumn{2}{c|}{$T_{p}$} &\multicolumn{2}{c|}{$T_{z}$} & \multicolumn{2}{c|}{Dir} \\
    %  \hline
       & Cora & Citeseer &  Pubmed & PPI &  Reddit \\
    %  \hline
    %  Task & • & • & • & • & • & • & •   \\
     \hline
     Type & Citation & Citation & Citation & Protein interaction & Communities  \\
     \hline
     \#Nodes & 2708 & 3327 & 19717 (1 graph) & 56944 (24 graphs) & 232965 (1 graph) \\
     \hline
     \#Edges  & 5429 & 4732 & 44338 & 818716 & 114615892   \\
     \hline
     \#Features/Nodes & 1433 & 3703 & 500 & 50 & 602   \\
     \hline
     \#Classes & 7 & 6 & 3 & 121(multilabel) & 41   \\
     \hline
     \#Training Nodes & 140 & 120 & 60 & 44906(20 graphs) & 153431    \\
     \hline
     \#Validation Nodes & 500 & 500 & 500 & 6513 (2 graphs) & 23831  \\
     \hline
     \#Testing Nodes  & 1000 & 1000 & 1000 & 5524 (2 graphs) & 55703   \\
     \hline
 \end{tabular}
 \end{adjustbox}
\end{table}


\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    Parameter Type & Grid \\
    \hline
    values nodes update rate & $0.05, 0.1, 0.5, 1.0$  \\
    Weight update learning rate & $1e-2$,$1e-3$,$1e-4$,$1e-5$ \\
    Number of GNN Layer & $2, 4$ \\
   Inference steps,T, & 12, 32, 50, 100\\
    PC synaptic weight update rate &  at the end of ,T, inference steps, and at every inference step\\
    aggregation functions  &  sum, add, max\\
    Graphsage sampling & 10, 25 for first and second GNN layer respectively\\
    \hline
  \end{tabular}
  \caption{Hyper-Parameter Search}\label{tab:hyperpar}
\end{table}




\section{Calibration Analysis: Confidence in Prediction} 
As deep networks tend to be overconfident even if they are wrong, we compared the confidence distribution of GPCNs with GCNs in Figure~\ref{fig:conf_distribution_cora},~\ref{fig:conf_distribution_citeseer}, and \ref{fig:conf_distribution}, where confidence is the maximum of the softmax of the model output. The result in this section correspond to the reported results in the body of the paper on calibration analysis in Section~\ref{sec:cal_analysis}. Both model are run for 300 epochs using the same parameters (i.e., learning rate on weights equal to 0.001) and we select the best model based on validation set for GCN. For GPCN, we select the best model based on best accuracy on validation set as well as lowest energy on training set as the energy minimization can be interpreted as likelihood maximisation. We consider energy while selecting the best model for evaluation because we discovered a high correlation between energy and robustness as we will demonstrate in the following section (see Figure~\ref{fig:energy_calibration}). Interestingly, the results on prediction distribution on provide another dimension to communicate the same results we witness in Section~\ref{sec:cal_analysis} using reliability diagrams. We see that on the prediction distribution on Cora dataset in Figure~\ref{fig:conf_distribution}, GPCNs are relatively less confident in their predictions, while GCN model is overly confident. Figure~\ref{fig:conf_distribution_citeseer} on Citeseer dataset similarly here shows that most prediction confidence of GCN model are less than 0.5, showing that GCN models are overly under-confident as we saw in the body of the paper. GPCNs models on the other hand provide a well behaved prediction confidence distribution on Citeseer. demonstrate that either GCN either is under-confident despite high performance accuracy or over-confident in the manner that is disproportional to its performance accuracy.


\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp/non_pc_confidence_distribution.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp/pc_confidence_distribution.pdf} }}%
    \caption{Histogram of prediction confidence distribution on Cora dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left: GCN. Right: GPCN.}%
    \label{fig:conf_distribution_cora}%
\end{figure}

\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp2/bp_confidence_distribution_cora_lr=0.01.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/pc_cite_seer_dist=0.001.pdf} }}%
    \caption{Histogram of prediction confidence distribution on Citeseer dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left diagram is for GCN while right diagram is ouput of GPCN.}%
    \label{fig:conf_distribution_citeseer}%
\end{figure}


\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp2/bp_confidence_distribution_pubmed_lr=0.001.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp2/pc_confidence_distribution_pubmed_lr=0.001.pdf} }}%
    \caption{Histogram of prediction confidence distribution on PubMed dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left: GCN. Right: GPCN.}%
    \label{fig:conf_distribution}%
\end{figure}

\subsection{Calibration Strengthening through Energy Minimization }

We observed a high positive correlation between calibration and training energy level, thus, we further investigated the role of energy to robustness and calibration of our learned representation. Unlike the standard predictive coding network, we observed, GPCN requires several inference steps to reach lowest training energy possible, i.e., this can seen as reaching local optimal of likelihood maximisation function. More importantly, we also observed that the lower the energy the better the calibration is, i.e., the better the model can estimate uncertainty in its prediction. Figure~\ref{fig:energy_calibration} on Cora dataset and Figure~\ref{fig:energy_calibration_citeseer} on CiteSeer dataset showcase this correlation. The plots on the left show that inference steps correlate to the energy level, i.e., the longer the inference is, the more likely that the model converge to a lower energy. The middle diagram and right diagrams, similarly, present the correlation between the inference steps and ECE and MCE, respectively, which from left diagrams, implies the correlation of energy level and ECE and MCE. We see that the lower the energy the better the calibration performance reached.

As it has been shown that calibration can be affected by learning rates \cite{guo2017calibration}, we track the ECE and MCE throughout training, and we see that as the lower the learning rate, the better and more stable calibration GPCN is able to attain based on ECE and MCE metrics (see Figure ~\ref{fig:ece_lr} and \ref{fig:mce_lr}).

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=12cm]{img/exp/TvsE.pdf}
    }
    \caption{Evaluation of the impact of energy on  calibration performance on Cora dataset (learning rate $= 0.001$). Left: Demonstrates that increasing inference steps leads to lower energy. Middle: Shows that the lower energy level determines expected error(ECE). Right: Also showcase, the correlation between energy and maximum calibration error(MCE)}
    \label{fig:energy_calibration}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=12cm]{img/exp/Citeseer_TvsE3.pdf}
    }
    \caption{Evaluation of the impact of energy on  calibration performance on CiteSeer dataset. Left: Demonstrates that increasing inference steps leads to lower energy. Middle: Shows that the lower energy level determines expected error(ECE). Right: Also showcase, the correlation between energy and maximum calibration error(MCE)}
    \label{fig:energy_calibration_citeseer}
\end{figure}




\begin{figure}
    \centering
{{\includegraphics[width=6.5cm]{img/exp2/bp_ece_plot.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp2/pc_ece_plot.pdf} }}%
    \caption{Evolution of expected calibration error (ECE) on test set during training on various learning rates (lr). Left: GCN. Right: GPCN.}%
    \label{fig:ece_lr}%
\end{figure}


\begin{figure}
    \centering
{{\includegraphics[width=6.5cm]{img/exp2/bp_mce_plot.pdf} }}%
    \qquad
{{\includegraphics[width=6.5cm]{img/exp2/pc_mce_plot.pdf} }}%
    \caption{Evolution of maximum calibration error (MCE) on test set during training on various learning rates (lr). Left: GCN. Right: GPCN.}%
    \label{fig:mce_lr}%
\end{figure}



\section{GPCN architecture}

Using a simple graph in Figure~\ref{fig:example_graph}, here, we demonstrate the idea of graph predictive coding as opposed to standard graph neural networks. In typical graph convolution network (GCN) \cite{welling2016semi} models, the node representation is obtained by the recursive aggregation of representations of its neighbours, after which a learned linear transformation and non-linear activation function are applied. After the $k_th$ round of aggregation (with $k$ denoting the number of GCN layer), the representation of a node reflects the underlying structure of its nearest neighbours within $k$ hops. Note that the GCN is one of the simplest GNN model, as the update function equates to only neighbourhood aggregation, that is why in Figure~\ref{fig:graph_mesage_passing}(left) we only depict the aggregate function as it captures the update function altogether. 

Our GPCN model (see Figure~\ref{fig:graph_mesage_passing}(right)) differs from the standard GNN in three aspects. First, node representation are not a mere result of neighborhood aggregation. Rather, each node has unique a neural state that is updated through energy-minimization using the theory of predictive coding described in the main body of this work. Specifically, each neighborhood aggregation at each hop, k,, pass through a predictive coding module that predicts the the incoming aggregated neighborhood representation. Second, GPCN has a different concept of what neighborhood messages are (see Figure~\ref{node_aggregation}). Rather than transmitting raw messages, it instead, forward residual error of the difference between the predicted representation and the aggregation  which reduce the dynamic range of the message being transmitted hence acting as low pass filter. Lastly, unlike the standard GNN that are trained using BP, where the update of weights corresponding to a given neighborhood are dependent, which create a large computation graphs, GPCN learning rules are local and the model weight are updated through energy minimization as we described in the methodology section.


\begin{figure}[H]
    \centering
    \includegraphics[width=3cm]{img/meth/example_graph.pdf}
    \caption{Example of graph that we use to illustrate the architecture.}
    \label{fig:example_graph}
\end{figure}

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/meth/inter_layer_pc_.pdf}
    }
    \caption{Distinction of Messaging propagation between standard GNNs (Left) and inter-layer GPCN (Right).}
    \label{fig:graph_mesage_passing}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/meth/Intra_layer_pc.pdf}
    }
    \caption{Distinction of the difference between message aggregation between standard GNNs and GPCN. Left: standard aggregation method, Right: intra-layer GPCN.}
    \label{fig:node_aggregation}
\end{figure}


\section{Additional Results on Evasion Attacks with Nettack}

Due to the page constraint, here we provide additional results we could not include in the main body of this paper. In particular, the foloowing plots demonstrate how both GCN and GPCN model perform under various perturbation budgets on the four types of attacks namely feature, structure, feature-structure, and indirect attacks. 

\textbf{1) Structure and Feature attack:}

Figure~\ref{fig:both_s_f_attack1} show that with only 2 perturbation on neighbourhood structure and features of victim nodes, the median classification margin approaches -1 on GCN model, while GPCN stays relatively robust and with more robustness on lower energy model(PCx3) where most of the victims nodes have positive classification margins, or in other worlds, they are not adversarially affect by the attack. This trend is even pronounced when perturbation rate is increase to five(Figure~\ref{fig:both_s_f_attack2}) and ten (Figure~\ref{fig:both_s_f_attack3}) where, except for outliers, margin of classification of all victims nodes falls to $-1$ for both GCN and PC model PCx3 stay lately more robust.


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/exp2_cora_pt_rate=2_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 2. On x-axis BP indicates GCN model, PC denotes GPCN model trained of 12 inference steps, and  PCx3 indicate GPCN trained using 36 inference steps, hence achieves lower training energy. }
    \label{fig:both_s_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/exp2_cora_pt_rate=5_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 5}
    \label{fig:both_s_f_attack2}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/both_energy_cora_pt_rate=10_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 10}
    \label{fig:both_s_f_attack3}
\end{figure}





\textbf{2) Feature attacks}.
Since feature attacks do not high affect GNNs as much as structure attacks, we peform, large corruption of features with perturbation rate of 1, 5, 10, 30, 50 and 100. We observe a similar trends where with a small perturbation on features does not affect the model, however, when perturbation rate become large our GPCN display unparalleled performance resisting the attacks. When perturbation rate is equal to 30 (see Figure~\ref{fig:only_f_attack30}, while GCN misclassifies around $70\%$ of the victim nodes, GPCN is still able to classify more than $70\%$ correctly  after perturbation. The highly superior performance is observed when perturbation rate is increase to $100$ in Figure~\ref{fig:only_f_attack100}, GCN mislassifies all victims nodes, while GPCN still classify correctly those nodes with most victims nodes in the upper quartile having positive classification margins.




\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=1_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 1}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=5_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 5}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=10_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 10}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=30_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 30}
    \label{fig:only_f_attack30}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=50_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 50}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=100_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 100}
    \label{fig:only_f_attack100}
\end{figure}







\textbf{3) Structure attacks}: GPCN also consistently outperforms GCN under structure-only attacks on number perturbation equal to 1, 2, 5 and 10 as it can be observed in Figure~\ref{fig:only_f_attack1},\ref{fig:only_f_attack2},\ref{fig:only_f_attack3},\ref{fig:only_f_attack5}, and \ref{fig:only_f_attack10}. 



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=1_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 1}
    \label{fig:only_f_attack1}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=2_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 2}
    \label{fig:only_f_attack2}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=3_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 3}
    \label{fig:only_f_attack3}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=5_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 5}
    \label{fig:only_f_attack5}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=10_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 10}
    \label{fig:only_f_attack10}
\end{figure}








\textbf{4) Indirect Attacks}:

For indirect attacks, we choose 5 influencing/neighboring nodes to attack for each victims node. We observe a similar trend that was found in the Nettack paper\cite{zugner2018adversarial}. We found that the influence or indirect attacks do not affects GNNs as much as other attacks as it can be witnessed from the box plots below. However, we also found that GPCN, especially one with smaller inference steps consistently outperforms all models, but all GPCN models are strictly better than GCN under all perturbations.

Note for Figure~\ref{fig:influence_attach_attack1}, \ref{fig:influence_attach_attack2}, and \ref{fig:influence_attach_attack3}, on x-axis, BP indicates GCN model, PC denotes GPCN model trained of 12 inference steps, and  PCx3 indicate GPCN trained using 36 inference steps, hence achieves lower training energy. The suffix 'untempered' indicates the performance of model on clean graph. To interpret the plots, a more robust model is one that retain a higher classification margins after the attacks.



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_struct_cora_pt_rate=2_att_s=True_att_f=False.mine.png}
    }
    \caption{Classification Margin Diagram on influence attack with perturbation equal to the degree of target node and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack1}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_struct_cora_pt_rate=5_att_s=True_att_f=False.mine.png}
    }
    \caption{Classification Margin Diagram on on influence attack with perturbation equal to the degree of target node and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack2}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_both_cora_pt_rate=1_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification Margin Diagram on influence attack with perturbation equal to 1 and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack3}
\end{figure}

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_both_cora_pt_rate=10_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification Margin Diagram on on influence attack with perturbation 10 and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack4}
\end{figure}









==> FINAL arXiv- Robust Graph Representation Learning via Predictive Coding/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Sections/Appendices.tex <==
\appendix

\begin{comment}
\section{Predictive Coding}
In both human and robotic learning, it entails the process of credit assignment, or identifying the steps in the processing chain that lead to an incorrect outcome. Understanding how the brain deals with the credit assignment issue is crucial for the fields of neuroscience and artificial intelligence. Many recent studies have looked to backpropagation, a staple of modern machine learning, as the answer\cite{lillicrap2020backpropagation}. However, the brain's ability to do backpropagation has been questioned, and it has been proposed that the brain's natural approach to learning may be more effective in terms of both time and energy optimization \cite{tsividis2017human}. Predictive coding mechanism has presented itself as an excellent candidate as is capable training neural networks through energy minimization and has been able to explain several brain functions.


Predictive coding is an influential theory of information processing in the brain. Predictive coding proposes that the brain has a world model or many world models in distinct brain areas where each model is a generative model that captures the cause of sensory input. New sensory inputs are then mapped to recognised causes. Minimizing the discrepancy between sensory data and predicted sensory inputs aids in determining which of multiple possible explanations best matches existing sensory data.

This idea has manifested itself independently in various areas and there are a number of distinct algorithms that have been proposed to realise it. In signal processing, linear predictive coding (LPC) was originally used in audio and speech processing for signal restoration, interpolation, compression and recognition \cite{spratling2017review}. LPC was initially employed in neuroscience to describe the function of the retina \cite{laughlin1990coding}, such as efficient coding, redundancy reduction, and normalisation. Later, numerous studies expanded on the notion of LPC to neural network based architecture to describe various cortical processes in the brain \cite{rao1999predictive, spratling2008predictive, friston2009free}. 

The training and inference mechanisms of predictive coding networks(PCNs) is in Appendix~\ref{sec:pc_formulation_sec}.

\section{Predictive Coding vs Back-propagation}

This section examines the differences between the backpropagation algorithm, the leading algorithm used to train artificial neural networks (ANNs), and inference learning (IL), which is one of the major method used to train predictive coding networks(PCNs).


\subsubsection{Training ANNs with BP}


% - Include a pc training algorithm in the background

A layer of an artificial neural network\cite{rumelhart1986learning} consists of a number of value nodes that mimic neurons. To further highlight the connection to PCNs, we invert the layer numbering scheme, assigning $0$ to the output layer and $l_{max}$ to the input layer (see \cite{song2020can} for additional details). Let nodes at $l^{th}$ layer be indicated by $\mathbf{h^l}$ vector, and for simplification we ignore the bias values. Then, the activation of $i$ neuron in in layer $l$ is calculated as follows:

\begin{equation}
\label{eqn:equ1}
  h_{i}^{l}=\sum_{j=1}^{|h^{l+1}|} w_{i, j}^{l+1} f\left(h_{j}^{l+1}\right)  
\end{equation}
where  $w_{i, j}^{l+1}$ denotes the synaptic weight connecting $l^{th}$ to ${l+1}^{th}$ layer.




\textbf{Learning}: Given the input vector $\mathbf{x}$ and true label vector $\mathbf{y}$, $\mathbf{h^{l_max}}$ is fixed to input vector $\mathbf{x}$ (i.e. $\mathbf{h^{l_max} = x}$). The output of the layer values are obtain through iterative application of Equation~\ref{eqn:equ1}, then the prediction error, E, is calculated using an objective function,  $\mathcal{L}$ (the most common loss function for classification and regression tasks are cross entropy and mean-squared error, respectively):


\begin{equation}
E=\mathcal{L}(\mathbf{y, h^0})
\end{equation}

Back-propagation algorithm\cite{rumelhart1986learning} essentially works by propagating the error gradient sequentially backward from the output layer through all network layers and utilises gradient descent algorithm to update the synaptic weight. The gradient with respect to a weight parameter,$w_{i, j}^{l+1}$, in layer ${l+1}$ is given by the following:

$$
\Delta w_{i, j}^{l+1}=-\eta \cdot \partial E / \partial w_{i, j}^{l+1}
$$

where $\eta$ denotes the learning rate. $i$ and $j$ subscripts represent in neurons in layer $l+1$ and $l$ respectively. 





\textbf{Prediction}: Given the input vector $\mathbf{x}$, $\mathbf{h^{l_max}}$ is fixed to input vector $x$ (i.e. $\mathbf{h^{l_max} = x}$), then the feedforward of the input signal through the network happen by recursively applying Equation~\ref{eqn:equ1}(like in training mode) and prediction are indicated by the output layer $0$. The top of Figure~\ref{fig:pc_bp} showcase this process.


% \subsubsection{Training PCNs with using inference learning}
% \label{sec:pc_formulation_sec}
% The architecture and learning method of Predictive Coding Networks(PCNs) is different from ANNs and back-propagation as illustrated in Figure~\ref{fig:pc_bp}. Like ANNs, PCNs have values nodes and synaptic weights, however, each values nodes is associated with additional error node, and are optimised using inference learning algorithm(see Algorithm~\ref{alg:cap}). In PCN architecture, a values node $h^{l}_{i, t}$ denotes neural activity of neuron $i$ at layer $l$ at time $t$ with corresponding prediction-error nodes $\varepsilon^{l}_{i, t}$. Inference learning\cite{whittington2017approximation} entail inferring the values of the hidden node through energy minimization. Different variations of IL such as Z-IL, Fa-Z-IL have been developed to make IL more efficient and give it full autonomy during training\cite{song2020can}.

% \textbf{Learning}: Given the input vector $\mathbf{x}$ and true label vector $\mathbf{y}$, $\mathbf{h^{l_max}}$ is fixed to input vector $x$ (i.e. $\mathbf{h^{l_max} = x}$) and output layer is fixed to true label values (i.e. $\mathbf{h^{0} = y}$). Unlike ANN that propagate the activity of nodes as directly, PCNs propagates the error node values, $\varepsilon__{i, t}^{l} $, i.e., the difference between the value nodes and the prediction of the node, $h^{l}_{i, t}$ and $\mu^{l}_{i, t}$, respectively.

% \begin{equation}
% \label{eqn:error_update}
% \mu_{i, t}^{l}=\sum_{j=1}^{|\mathbf{h^{l+1}}|} w_{i, j}^{l+1} f\left(x_{j, t}^{l+1}\right) \text { and } \varepsilon_{i, t}^{l}=h_{i, t}^{l}-\mu_{i, t}^{l} \text {, }
% \end{equation}

% where  $w_{i, j}^{l+1}$ denotes the synaptic weight  beween  node $i$ at layer $l$ and node $j$ at layer $l+1$.

% \textbf{Energy Minimization}. As PCNs are energy-based models, the training happen through minimization of the global energy in each layer. Under the assumption of Gaussian distribution with identify covariance, the energy,$F_{t}$ function of PCNs can be derived simply as the sum of errors of prediction-error nodes in the network \cite{whittington2017approximation}:

% $$
% F_{t}=\frac{1}{2} \sum_{i, l}\left(\varepsilon_{i, t}^{l}\right)^{2}
% $$


% Minimizing this function brings each value node $h^{l}_{i, t}$ closer to its correct prediction. Inference, in this case, describes this process of reducing energy function, $Ft$,via tweaking $h_{i, t}^{l}$ to match $\mu_{i, t}^{l}$. This process is described by the following equation dynamics:

% \begin{equation}
% \label{eqn:x_update}
% \Delta h_{i, t}^{l}= \begin{cases}0 & \text { if } l=l_max \\ \gamma \cdot\left(-\varepsilon_{i, t}^{l}+f^{\prime}\left(h_{i, t}^{l}\right) \sum_{k=1}^{n^{l-1}} \varepsilon_{k, t}^{l-1} w_{k, i}^{l}\right) & \text { if } 0<l<l_max \\ \gamma \cdot\left(-\varepsilon_{i, t}^{l}\right) & \text { if } l=0,\end{cases}
% \end{equation}


% where $\gamma$ is the integration step

% Using to the Equation~\ref{eqn:x_update}, the value nodes are updated until convergence, or until inference steps reaches $T$ iterations. Following the inference step, a single weight update is executed to further reduce the residual errors $E$. Then, the weights, $W$, are modified in order to minimise the same objective function $F_t$, using the following equation:

% \begin{equation}
% \label{eqn:w_update}
% \Delta w_{i, j}^{l+1}=-\alpha \cdot \partial F_{t} / \partial w_{i, j}^{l+1}=\alpha \cdot \varepsilon_{i, t}^{l} f\left(h_{j, t}^{l+1}\right)
% \end{equation}

% This inference learning process is described in Algorithm~\ref{alg:cap}.



% \textbf{Prediction}. For acyclic fully-connected network, the prediction stage is similar to ANNs, which is simply a single feed-forward pass of sensory signals through the network. Because the output is usually unconstrained, the inference process optimise the weights so that error nodes decay to zero as $t \rightarrow \infty$. Thus, the values nodes, $h_{i, t}^{l}$, converge to the prediction values, $\mu_{i, t}^{l}$. For architecture with complex topologies, a inference process is necessary during prediction stage\cite{salvatori2022learning}.



% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{img/pc_bp_diagram.pdf}
%     \caption{Neural implementation of Back-propagation (top) and predictive coding (bottom). The blue lines refers to  Equation~\ref{eqn:equ1} and Equation~\ref{eqn:error_update} ANN and PCN, respectively,  and the red line refers to Equation~\ref{eqn:x_update} for PCN .}
%     \label{fig:pc_bp}
% \end{figure}


% \begin{algorithm}
% \caption{Learning one training pair ($x$, $y$) (presented for the duration T, i.e., inference steps) with IL (This algorithm was adapted from \cite{song2020can})}\label{alg:cap}
% \begin{algorithmic}[1]
% \Require $h_{0 \max }^l$ is fixed to $y, \bar{h}_0^0$ is fixed to $x$

% \For {\texttt{ t=0 \text { to } T} }
% \For {\texttt{each neuron i in each level l} }

% \State \texttt{Update $h_{i, t}^l$ to minimize $F_t$ using Equation~\ref{eqn:x_update}}
% \State \texttt{Update each $w_{i, j}^{l+1}$ to minimize $F_t$ using Equation~\ref{eqn:w_update}}

   

% \EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}


% \textbf{Biological plausibility}. In additional to the ability of predictive coding to explain many neuro-biological phenomena,  one of the attractive of predictive coding networks is that they rely on local computation which explain local plasticity of synaptic weights. In contrast to BP,  Eqs~\ref{eqn:error_update}, \ref{eqn:x_update}, and \ref{eqn:w_update} in IL rely on local information. An external signal is still required to terminate inference at time $t=T$ and initiate the weights update, thus the full autonomy required for biological plausibility is not fully realised. However, an extension of IL known as fully autonomous zero-divergent IL (Fa-Z-IL) realise full autonomy\cite{song2020can}.
\end{comment}



\section{Details on evaluation metrics}

In this section, we explain the metrics used in the main body of this work in more detail. We employ scalar quantification metrics, such as expected calibration error (ECE) and maximum calibration error, together with visual tools, such as reliability diagrams and confidence distribution histograms \citep{guo2017calibration} and classification margin diagrams \citep{dai2018adversarial} to evaluate model calibration.

The term `confidence calibration` is used to describe the ability of a model to produce probability estimations that are accurate reflections of the correct likelihood an event, which is imperative especially in real-world applications. Considering a $K$-class classification task, let  $X \in \mathcal{X}$ and $Y \in \mathcal{Y}=\{1, \ldots, K\}$ be input and true ground truth label random variables, respectively. Let $\hat{Y}$ denote a class prediction and $\hat{P}$ be its associated confidence, i.e. probability of correctness. We would like the confidence estimate $\hat{P}$ to be calibrated, which intuitively means that $\hat{P}$ represents a true probability. The perfect calibration can be described as follows:
%
\begin{equation}
\label{eqn:calibration}
    \mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)=p, \quad \forall p \in[0,1]
\end{equation}
%
\textbf{ECE} captures the notion of average miscalibration in a single number, and can be obtained by the expected difference between  accuracy and confiedence of the model: $
\underset{\hat{P}}{\mathbb{E}}[|\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)-p|]
$




\textbf{MCE} is much crucial in safety-, security-critical settings, as it quantifies worst-case expected miscalibration: $
\max _{p \in[0,1]}|\mathbb{P}(\hat{Y}=Y \mid \hat{P}=p)-p| .
$

\textbf{Reliability diagrams} are visual representation tools for model calibration as equation~\ref{eqn:calibration} is intractable because  $\hat{P}$ is a continuous random variable. They characterise the average accuracy level inside a points that feels into a given confidence level bin (see \cite{} for more details on formulation of the the above metrics).

\textbf{Classification margin} is simply the difference between the model output probability of the ground truth class and the model probability of the predicted most-likely class, i.e.,the probability of the best second class. Thus, this metric is between $-1$ and $1$, where values close to $-1$ indicate that a model is overconfident in wrong predictions and values closer to $1$ indicate that the model is confidence in its correct prediction. In our reported class margin diagrams,  we average these values over many samples and repeated trials with different random seeds to draw box-plot diagrams of our results. 


\section{Reproducibility}

We use standard splits on all datasets. We report the average results of 5 runs on different seeds; the hyper-parameters are selected using the validation set. Following the results from original papers on baseline models, we evaluate our model on 2 GNN layers. The models are trained for 300 epochs on citation graphs and 50 epochs on PPI. We also use Adam optimiser. The reported results on calibration analysis were performed on initial learning rate of 0.001 for both GCN and GPCN as it provided best performances for both models. For adversarial attacks, we set initial learning rate to 0.01 and epochs to 200 to compare our results to other works. For general performance experiment, we use grid search for hyper-parameters as described in Table~\ref{tab:hyperpar}. Inductive tasks were trained using GCN version of GraphSage \citep{hamilton2017inductive} with neighborhood sample size of 25 and 10 for first and second GNN layer, respectively (see \cite{hamilton2017inductive} for more details). 


Our experiments are performed using Pytorch Geometric library \cite{fey2019fast}. In order to do an extensive experiment, we build on GraphGym \cite{you2020design}, a research platform for designing and evaluating GNNs, and we seamlessly integrate it with predictive coding learning algorithm. In addition, we employ another Pytorch library for adversarial attacks and defenses known as Deeprobust \cite{li2020deeprobust} for various type of adversarial attacks we perform on graphs.



\subsection{Datasets}
\begin{table}[H]
    \caption{An overview of the data sets used in our experiments }\label{tab:datasets}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{*{7}{|c}|}\hline
    %   • &\multicolumn{8}{c|}{West Hebrides} \\
    %  \hline
    %  • & \multicolumn{2}{c|}{$H_{s}$} &\multicolumn{2}{c|}{$T_{p}$} &\multicolumn{2}{c|}{$T_{z}$} & \multicolumn{2}{c|}{Dir} \\
    %  \hline
       & Cora & Citeseer &  Pubmed & PPI &  Reddit \\
    %  \hline
    %  Task & • & • & • & • & • & • & •   \\
     \hline
     Type & Citation & Citation & Citation & Protein interaction & Communities  \\
     \hline
     \#Nodes & 2708 & 3327 & 19717 (1 graph) & 56944 (24 graphs) & 232965 (1 graph) \\
     \hline
     \#Edges  & 5429 & 4732 & 44338 & 818716 & 114615892   \\
     \hline
     \#Features/Nodes & 1433 & 3703 & 500 & 50 & 602   \\
     \hline
     \#Classes & 7 & 6 & 3 & 121(multilabel) & 41   \\
     \hline
     \#Training Nodes & 140 & 120 & 60 & 44906(20 graphs) & 153431    \\
     \hline
     \#Validation Nodes & 500 & 500 & 500 & 6513 (2 graphs) & 23831  \\
     \hline
     \#Testing Nodes  & 1000 & 1000 & 1000 & 5524 (2 graphs) & 55703   \\
     \hline
 \end{tabular}
 \end{adjustbox}
\end{table}


\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    Parameter Type & Grid \\
    \hline
    values nodes update rate & $0.05, 0.1, 0.5, 1.0$  \\
    Weight update learning rate & $1e-2$,$1e-3$,$1e-4$,$1e-5$ \\
    Number of GNN Layer & $2, 4$ \\
   Inference steps,T, & 12, 32, 50, 100\\
    PC synaptic weight update rate &  at the end of ,T, inference steps, and at every inference step\\
    aggregation functions  &  sum, add, max\\
    Graphsage sampling & 10, 25 for first and second GNN layer respectively\\
    \hline
  \end{tabular}
  \caption{Hyper-Parameter Search}\label{tab:hyperpar}
\end{table}




\section{Calibration Analysis: Confidence in Prediction} 
As deep networks tend to be overconfident even if they are wrong, we compared the confidence distribution of GPCNs with GCNs in Figure~\ref{fig:conf_distribution_cora},~\ref{fig:conf_distribution_citeseer}, and \ref{fig:conf_distribution}, where confidence is the maximum of the softmax of the model output. The result in this section correspond to the reported results in the body of the paper on calibration analysis in Section~\ref{sec:cal_analysis}. Both model are run for 300 epochs using the same parameters (i.e., learning rate on weights equal to 0.001) and we select the best model based on validation set for GCN. For GPCN, we select the best model based on best accuracy on validation set as well as lowest energy on training set as the energy minimization can be interpreted as likelihood maximisation. We consider energy while selecting the best model for evaluation because we discovered a high correlation between energy and robustness as we will demonstrate in the following section (see Figure~\ref{fig:energy_calibration}). Interestingly, the results on prediction distribution on provide another dimension to communicate the same results we witness in Section~\ref{sec:cal_analysis} using reliability diagrams. We see that on the prediction distribution on Cora dataset in Figure~\ref{fig:conf_distribution}, GPCNs are relatively less confident in their predictions, while GCN model is overly confident. Figure~\ref{fig:conf_distribution_citeseer} on Citeseer dataset similarly here shows that most prediction confidence of GCN model are less than 0.5, showing that GCN models are overly under-confident as we saw in the body of the paper. GPCNs models on the other hand provide a well behaved prediction confidence distribution on Citeseer. demonstrate that either GCN either is under-confident despite high performance accuracy or over-confident in the manner that is disproportional to its performance accuracy.


\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp/non_pc_confidence_distribution.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp/pc_confidence_distribution.pdf} }}%
    \caption{Histogram of prediction confidence distribution on Cora dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left: GCN. Right: GPCN.}%
    \label{fig:conf_distribution_cora}%
\end{figure}

\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp2/bp_confidence_distribution_cora_lr=0.01.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/pc_cite_seer_dist=0.001.pdf} }}%
    \caption{Histogram of prediction confidence distribution on Citeseer dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left diagram is for GCN while right diagram is ouput of GPCN.}%
    \label{fig:conf_distribution_citeseer}%
\end{figure}


\begin{figure}[H]
    \centering
    {{\includegraphics[width=6.5cm]{img/exp2/bp_confidence_distribution_pubmed_lr=0.001.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp2/pc_confidence_distribution_pubmed_lr=0.001.pdf} }}%
    \caption{Histogram of prediction confidence distribution on PubMed dataset. The x-axis indicates the confidence of the model on the samples, and y-axis is the count on a normal scale of data points that fall into a given confidence bin. Left: GCN. Right: GPCN.}%
    \label{fig:conf_distribution}%
\end{figure}

\subsection{Calibration Strengthening through Energy Minimization }

We observed a high positive correlation between calibration and training energy level, thus, we further investigated the role of energy to robustness and calibration of our learned representation. Unlike the standard predictive coding network, we observed, GPCN requires several inference steps to reach lowest training energy possible, i.e., this can seen as reaching local optimal of likelihood maximisation function. More importantly, we also observed that the lower the energy the better the calibration is, i.e., the better the model can estimate uncertainty in its prediction. Figure~\ref{fig:energy_calibration} on Cora dataset and Figure~\ref{fig:energy_calibration_citeseer} on CiteSeer dataset showcase this correlation. The plots on the left show that inference steps correlate to the energy level, i.e., the longer the inference is, the more likely that the model converge to a lower energy. The middle diagram and right diagrams, similarly, present the correlation between the inference steps and ECE and MCE, respectively, which from left diagrams, implies the correlation of energy level and ECE and MCE. We see that the lower the energy the better the calibration performance reached.

As it has been shown that calibration can be affected by learning rates \cite{guo2017calibration}, we track the ECE and MCE throughout training, and we see that as the lower the learning rate, the better and more stable calibration GPCN is able to attain based on ECE and MCE metrics (see Figure ~\ref{fig:ece_lr} and \ref{fig:mce_lr}).

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=12cm]{img/exp/TvsE.pdf}
    }
    \caption{Evaluation of the impact of energy on  calibration performance on Cora dataset (learning rate $= 0.001$). Left: Demonstrates that increasing inference steps leads to lower energy. Middle: Shows that the lower energy level determines expected error(ECE). Right: Also showcase, the correlation between energy and maximum calibration error(MCE)}
    \label{fig:energy_calibration}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=12cm]{img/exp/Citeseer_TvsE3.pdf}
    }
    \caption{Evaluation of the impact of energy on  calibration performance on CiteSeer dataset. Left: Demonstrates that increasing inference steps leads to lower energy. Middle: Shows that the lower energy level determines expected error(ECE). Right: Also showcase, the correlation between energy and maximum calibration error(MCE)}
    \label{fig:energy_calibration_citeseer}
\end{figure}




\begin{figure}
    \centering
{{\includegraphics[width=6.5cm]{img/exp2/bp_ece_plot.pdf} }}%
    \qquad
    {{\includegraphics[width=6.5cm]{img/exp2/pc_ece_plot.pdf} }}%
    \caption{Evolution of expected calibration error (ECE) on test set during training on various learning rates (lr). Left: GCN. Right: GPCN.}%
    \label{fig:ece_lr}%
\end{figure}


\begin{figure}
    \centering
{{\includegraphics[width=6.5cm]{img/exp2/bp_mce_plot.pdf} }}%
    \qquad
{{\includegraphics[width=6.5cm]{img/exp2/pc_mce_plot.pdf} }}%
    \caption{Evolution of maximum calibration error (MCE) on test set during training on various learning rates (lr). Left: GCN. Right: GPCN.}%
    \label{fig:mce_lr}%
\end{figure}



\section{GPCN architecture}

Using a simple graph in Figure~\ref{fig:example_graph}, here, we demonstrate the idea of graph predictive coding as opposed to standard graph neural networks. In typical graph convolution network (GCN) \cite{welling2016semi} models, the node representation is obtained by the recursive aggregation of representations of its neighbours, after which a learned linear transformation and non-linear activation function are applied. After the $k_th$ round of aggregation (with $k$ denoting the number of GCN layer), the representation of a node reflects the underlying structure of its nearest neighbours within $k$ hops. Note that the GCN is one of the simplest GNN model, as the update function equates to only neighbourhood aggregation, that is why in Figure~\ref{fig:graph_mesage_passing}(left) we only depict the aggregate function as it captures the update function altogether. 

Our GPCN model (see Figure~\ref{fig:graph_mesage_passing}(right)) differs from the standard GNN in three aspects. First, node representation are not a mere result of neighborhood aggregation. Rather, each node has unique a neural state that is updated through energy-minimization using the theory of predictive coding described in the main body of this work. Specifically, each neighborhood aggregation at each hop, k,, pass through a predictive coding module that predicts the the incoming aggregated neighborhood representation. Second, GPCN has a different concept of what neighborhood messages are (see Figure~\ref{node_aggregation}). Rather than transmitting raw messages, it instead, forward residual error of the difference between the predicted representation and the aggregation  which reduce the dynamic range of the message being transmitted hence acting as low pass filter. Lastly, unlike the standard GNN that are trained using BP, where the update of weights corresponding to a given neighborhood are dependent, which create a large computation graphs, GPCN learning rules are local and the model weight are updated through energy minimization as we described in the methodology section.


\begin{figure}[H]
    \centering
    \includegraphics[width=3cm]{img/meth/example_graph.pdf}
    \caption{Example of graph that we use to illustrate the architecture.}
    \label{fig:example_graph}
\end{figure}

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/meth/inter_layer_pc_.pdf}
    }
    \caption{Distinction of Messaging propagation between standard GNNs (Left) and inter-layer GPCN (Right).}
    \label{fig:graph_mesage_passing}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/meth/Intra_layer_pc.pdf}
    }
    \caption{Distinction of the difference between message aggregation between standard GNNs and GPCN. Left: standard aggregation method, Right: intra-layer GPCN.}
    \label{fig:node_aggregation}
\end{figure}


\section{Additional Results on Evasion Attacks with Nettack}

Due to the page constraint, here we provide additional results we could not include in the main body of this paper. In particular, the foloowing plots demonstrate how both GCN and GPCN model perform under various perturbation budgets on the four types of attacks namely feature, structure, feature-structure, and indirect attacks. 

\textbf{1) Structure and Feature attack:}

Figure~\ref{fig:both_s_f_attack1} show that with only 2 perturbation on neighbourhood structure and features of victim nodes, the median classification margin approaches -1 on GCN model, while GPCN stays relatively robust and with more robustness on lower energy model(PCx3) where most of the victims nodes have positive classification margins, or in other worlds, they are not adversarially affect by the attack. This trend is even pronounced when perturbation rate is increase to five(Figure~\ref{fig:both_s_f_attack2}) and ten (Figure~\ref{fig:both_s_f_attack3}) where, except for outliers, margin of classification of all victims nodes falls to $-1$ for both GCN and PC model PCx3 stay lately more robust.


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/exp2_cora_pt_rate=2_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 2. On x-axis BP indicates GCN model, PC denotes GPCN model trained of 12 inference steps, and  PCx3 indicate GPCN trained using 36 inference steps, hence achieves lower training energy. }
    \label{fig:both_s_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/exp2_cora_pt_rate=5_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 5}
    \label{fig:both_s_f_attack2}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/both_energy_cora_pt_rate=10_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on both features and structure when perturbation rate equal to 10}
    \label{fig:both_s_f_attack3}
\end{figure}





\textbf{2) Feature attacks}.
Since feature attacks do not high affect GNNs as much as structure attacks, we peform, large corruption of features with perturbation rate of 1, 5, 10, 30, 50 and 100. We observe a similar trends where with a small perturbation on features does not affect the model, however, when perturbation rate become large our GPCN display unparalleled performance resisting the attacks. When perturbation rate is equal to 30 (see Figure~\ref{fig:only_f_attack30}, while GCN misclassifies around $70\%$ of the victim nodes, GPCN is still able to classify more than $70\%$ correctly  after perturbation. The highly superior performance is observed when perturbation rate is increase to $100$ in Figure~\ref{fig:only_f_attack100}, GCN mislassifies all victims nodes, while GPCN still classify correctly those nodes with most victims nodes in the upper quartile having positive classification margins.




\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=1_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 1}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=5_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 5}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=10_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 10}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=30_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 30}
    \label{fig:only_f_attack30}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=50_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 50}
    \label{fig:only_f_attack1}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/features_cora_pt_rate=100_att_s=False_att_f=True.mine.png}
    }
    \caption{Classification margin diagram of targeted attack on features when perturbation rate equal to 100}
    \label{fig:only_f_attack100}
\end{figure}







\textbf{3) Structure attacks}: GPCN also consistently outperforms GCN under structure-only attacks on number perturbation equal to 1, 2, 5 and 10 as it can be observed in Figure~\ref{fig:only_f_attack1},\ref{fig:only_f_attack2},\ref{fig:only_f_attack3},\ref{fig:only_f_attack5}, and \ref{fig:only_f_attack10}. 



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=1_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 1}
    \label{fig:only_f_attack1}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=2_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 2}
    \label{fig:only_f_attack2}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=3_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 3}
    \label{fig:only_f_attack3}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=5_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 5}
    \label{fig:only_f_attack5}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp/struct_cora_pt_rate=10_att_s=True_att_f=False.mine.png}}
    \caption{Classification margin diagram of targeted attack on structure when perturbation rate equal to 10}
    \label{fig:only_f_attack10}
\end{figure}








\textbf{4) Indirect Attacks}:

For indirect attacks, we choose 5 influencing/neighboring nodes to attack for each victims node. We observe a similar trend that was found in the Nettack paper\cite{zugner2018adversarial}. We found that the influence or indirect attacks do not affects GNNs as much as other attacks as it can be witnessed from the box plots below. However, we also found that GPCN, especially one with smaller inference steps consistently outperforms all models, but all GPCN models are strictly better than GCN under all perturbations.

Note for Figure~\ref{fig:influence_attach_attack1}, \ref{fig:influence_attach_attack2}, and \ref{fig:influence_attach_attack3}, on x-axis, BP indicates GCN model, PC denotes GPCN model trained of 12 inference steps, and  PCx3 indicate GPCN trained using 36 inference steps, hence achieves lower training energy. The suffix 'untempered' indicates the performance of model on clean graph. To interpret the plots, a more robust model is one that retain a higher classification margins after the attacks.



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_struct_cora_pt_rate=2_att_s=True_att_f=False.mine.png}
    }
    \caption{Classification Margin Diagram on influence attack with perturbation equal to the degree of target node and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack1}
\end{figure}



\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_struct_cora_pt_rate=5_att_s=True_att_f=False.mine.png}
    }
    \caption{Classification Margin Diagram on on influence attack with perturbation equal to the degree of target node and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack2}
\end{figure}


\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_both_cora_pt_rate=1_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification Margin Diagram on influence attack with perturbation equal to 1 and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack3}
\end{figure}

\begin{figure}[H]
    \centering
    \makebox[\textwidth]{
    \includegraphics[width=\textwidth]{img/exp2/influence_both_cora_pt_rate=10_att_s=True_att_f=True.mine.png}
    }
    \caption{Classification Margin Diagram on on influence attack with perturbation 10 and 5 influencing neighboring nodes}
    \label{fig:influence_attach_attack4}
\end{figure}








